Multi-Task Instruction Tuning of LLaMa for Specific Scenarios: A Preliminary Study on Writing Assistance

Proprietary Large Language Models (LLMs), such as ChatGPT, have garnered significant attention due to their exceptional capabilities in handling a diverse range of tasks. Recent studies demonstrate that open-sourced smaller foundational models, such as 7B-size LLaMA, can also display remarkable proficiency in tackling diverse tasks when fine-tuned using instruction-driven data. In this work, we investigate a practical problem setting where the primary focus is on one or a few particular tasks rather than general-purpose instruction following, and explore whether LLMs can be beneficial and further improved for such targeted scenarios. We choose the writing-assistant scenario as the testbed, which includes seven writing tasks. We collect training data for these tasks, reframe them in an instruction-following format, and subsequently refine the LLM, specifically LLaMA, via instruction tuning. Experimental results show that fine-tuning LLaMA on writing instruction data significantly improves its ability on writing tasks. We also conduct more experiments and analyses to offer insights for future work on effectively fine-tuning LLaMA for specific scenarios. Finally, we initiate a discussion regarding the necessity of employing LLMs for only one targeted task, taking into account the efforts required for tuning and the resources consumed during deployment.

==> figures/annotation_workflow.tex <==
\begin{figure}[tp!]
\centering
\includegraphics[scale=0.4]{figures/annotation_workflow.pdf}
\caption{The construction procedure of NaSGEC.}
\label{fig:anno:flow}
\end{figure}


==> figures/annotator_interface.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.3]{figures/annotator_interface.pdf}
\caption{Our annotation interface.}
\label{fig:anno:inter}
\end{figure}


==> figures/data_source.tex <==
\begin{figure*}[h]
\centering
\includegraphics[scale=0.57]{figures/data_source.pdf}
\caption{The screenshots of data sources for our 3 domains.}
\label{fig:data:source}
\end{figure*}

==> figures/review_interface.tex <==
\begin{figure}[h]
\centering
\includegraphics[scale=0.3]{figures/review_interface.pdf}
\caption{Our review interface.}
\label{fig:review:inter}
\end{figure}
